P4Testgen: An Extensible Test Oracle For P4

We present P4Testgen, a test oracle for the P4$_{16}$ language. P4Testgen supports automatic test generation for any P4 target and is designed to be extensible to many P4 targets. It models the complete semantics of the target's packet-processing pipeline including the P4 language, architectures and externs, and target-specific extensions. To handle non-deterministic behaviors and complex externs (e.g., checksums and hash functions), P4Testgen uses taint tracking and concolic execution. It also provides path selection strategies that reduce the number of tests required to achieve full coverage. We have instantiated P4Testgen for the V1model, eBPF, PNA, and Tofino P4 architectures. Each extension required effort commensurate with the complexity of the target. We validated the tests generated by P4Testgen by running them across the entire P4C test suite as well as the programs supplied with the Tofino P4 Studio. Using the tool, we have also confirmed 25 bugs in mature, production toolchains for BMv2 and Tofino.

==> Makefile <==
# Put user-specific changes in your own Makefile.user.
# Make will silently continue if that file does not exist.
-include Makefile.user

TARGET   = main
TARGET_BIB   = main

STYFILES = $(wildcard *.sty) $(wildcard *.cls)

PSTOPDF ?= pstopdf

.SUFFIXES:	.plot .eps .pdf

all: $(TARGET).pdf

draft: $(TARGET).pdf
	mkdir -p drafts
	cp $(TARGET).pdf drafts/draft-$(shell date "+%Y-%m-%d")-$(shell cat *.tex | shasum | head -c 8).pdf

html: $(TARGET).html

# used to launch editor that works with synctex etc
# see: https://github.com/mhinz/neovim-remote
editor:
	NVIM_LISTEN_ADDRESS=/tmp/nvimsocket nvim

#copy over main file from craig's related work file
EXTRA_DEPS := \
	 main.bib

OUTSIDE_BIB := ../main.bib
#this rule does nothing on purpose so this works on systems without the outside bib
# on systems with such a file, it copies it over
$(OUTSIDE_BIB):
	# bib creation no-op
main.bib: $(OUTSIDE_BIB)
	if [ -f $(OUTSIDE_BIB) ]; then cp $(OUTSIDE_BIB) . ; fi

$(TARGET).html: ${PDF_FIGURES} $(TARGET).bbl $(wildcard *.tex) $(STYFILES)  $(EXTRA_DEPS)
	htlatex -shell-escape $(TARGET).tex
	htlatex -shell-escape $(TARGET).tex

$(TARGET).pdf: ${PDF_FIGURES} $(TARGET).bbl $(wildcard *.tex) $(STYFILES)  $(EXTRA_DEPS)
	pdflatex -shell-escape $(TARGET).tex
	pdflatex -shell-escape $(TARGET).tex

$(TARGET).aux: $(TARGET).tex $(wildcard *.tex)
	pdflatex -shell-escape $(TARGET)

$(TARGET).bbl: $(TARGET_BIB).bib $(TARGET).aux
	pdflatex -shell-escape $(TARGET).tex
	bibtex $(TARGET)

tags: TAGS
.PHONY: tags TAGS html
TAGS:
	etags `latex-process-inputs --list usenix.tex`

clean:
	rm -f $(TARGET).pdf
	rm -f $(TARGET).log
	rm -f $(TARGET).blg
	rm -f $(TARGET).aux
	rm -f $(TARGET).bbl
	rm -f $(TARGET).dvi
	rm -f $(TARGET).out
	rm -f $(TARGET).toc
	rm -f $(TARGET).html $(TARGET).css $(TARGET).4ct $(TARGET).4tc \
		$(TARGET).xref $(TARGET).idv $(TARGET).lg $(TARGET).tmp \
		$(TARGET)*.html

